BS-Breath: Respiration Sensing with Cell-free Massive MIMO

This paper demonstrates the feasibility of respiration pattern estimation utilizing a communication-centric cellfree massive MIMO OFDM Base Station (BS). The sensing target is typically positioned near the User Equipment (UE), which transmits uplink pilots to the BS. Our results demonstrate the potential of massive MIMO systems for accurate and reliable vital sign estimation. Initially, we adopt a single antenna sensing solution that combines multiple subcarriers and a breathing projection to align the 2D complex breathing pattern to a single displacement dimension. Then, Weighted Antenna Combining (WAC) aggregates the 1D breathing signals from multiple antennas. The results demonstrate that the combination of space-frequency resources specifically in terms of subcarriers and antennas yields higher accuracy than using only a single antenna or subcarrier. Our results significantly improved respiration estimation accuracy by using multiple subcarriers and antennas. With WAC, we achieved an average correlation of 0.8 with ground truth data, compared to 0.6 for single antenna or subcarrier methods, a 0.2 correlation increase. Moreover, the system produced perfect breathing rate estimates. These findings suggest that the limited bandwidth (18 MHz in the testbed) can be effectively compensated by utilizing spatial resources, such as distributed antennas.

==> 02_related_work.tex <==
\section{related work}

\begin{enumerate}

    \item wifi sensing challenge, In practice, becuase of the Carrier-sense multiple access with collision avoidance (CSMA/CA) of Wi-Fi, multi-user scenarios typically cause a much lower and very irregular frame arrival rate per link. While radar sensing requires a regularly spaced channel for accurate estimation, such as micro-doppler estimation. To reconstuct the high quality signatures from the irregular spaced channel, \cite{} formulated this challenge as sparse recovery problem.
    
    \item multi-person sensing challenge, sub-6GHz RF sensing faces a major challenge in the presence of multiple persons, because of the limited bandwidth of Wi-Fi/BS fails to provide a sufficient range resolution to seperate multiple subjects. \cite{} trying to tackle this challenge utilizing blind source separation algorithm, while which requires the prior knowledge of number of subjects, which is not practical. \cite{} solve this problem with near-field channel, The principle behind MUSE-Fi is that, given a Wi-Fi device (e.g., smartphone) very close to a subject, the near-field channel variation caused by the subject significantly overwhelms variations caused by other distant subjects. Consequently, focusing on the channel state information (CSI) carried by the traffic in and out of this device naturally allows for physically separating multiple subjects.
    
    \item interfering challenge, most of RF respiration sensing studies are limited to certain scenarios without addressing the motion interference from other individuals. \cite{} tackle the challenge by separating targets and interfering individual with beam control strategy. However \cite{} assumes 
    
\end{enumerate}
